Mitigating Evasion Attacks in Federated Learning-Based Signal Classifiers

Recent interest in leveraging federated learning (FL) for radio signal classification (SC) tasks has shown promise but FL-based SC remains susceptible to model poisoning adversarial attacks. These adversarial attacks mislead the ML model training process, damaging ML models across the network and leading to lower SC performance. In this work, we seek to mitigate model poisoning adversarial attacks on FL-based SC by proposing the Underlying Server Defense of Federated Learning (USD-FL). Unlike existing server-driven defenses, USD-FL does not rely on perfect network information, i.e., knowing the quantity of adversaries, the adversarial attack architecture, or the start time of the adversarial attacks. Our proposed USD-FL methodology consists of deriving logits for devices' ML models on a reserve dataset, comparing pair-wise logits via 1-Wasserstein distance and then determining a time-varying threshold for adversarial detection. As a result, USD-FL effectively mitigates model poisoning attacks introduced in the FL network. Specifically, when baseline server-driven defenses do have perfect network information, USD-FL outperforms them by (i) improving final ML classification accuracies by at least 6%, (ii) reducing false positive adversary detection rates by at least 10%, and (iii) decreasing the total number of misclassified signals by over 8%. Moreover, when baseline defenses do not have perfect network information, we show that USD-FL achieves accuracies of approximately 74.1% and 62.5% in i.i.d. and non-i.i.d. settings, outperforming existing server-driven baselines, which achieve 52.1% and 39.2% in i.i.d. and non-i.i.d. settings, respectively.

==> atks_resources.tex <==
{\color{blue} for resources see: (i)\text{https://hongyanz.github.io/slides/cs886_s22_Lecture3.pdf}, (ii)\text{https://github.com/cleverhans-lab/cleverhans/tree/master/cleverhans/tf2/attacks}}

==> defense_init.tex <==
\section{The defense}

High level explanation of the 3-step defense algorithm 
\begin{enumerate}
    \item Identification of adversaries
    \item Quarantine of adversaries
    \item Aggregation of ML models from "good" devices only
\end{enumerate}

This is a novel networking-driven defense, rather than a data-driven defense as commonly seen in centralized defense methods. In order to enable such a method, a few new things need to be done:

\textbf{Preliminary steps:}
\begin{enumerate}
    \item Keep a small subset of training data - called a reserve dataset, this reserve dataset will not be at any device! All labels should be equally (or fairly equally) represented in this reserve dataset. 
    \item Using the reserve dataset, pre-train an ML model. Then when training starts at each "device", it starts from this pre-trained ML model.
\end{enumerate}

\textbf{Identification of adversaries}
\begin{enumerate}
    \item After X rounds of training, we need to try to aggregate these ML models. 
    \item To identify adversaries, we test each local ML model on the reserve dataset. 
    \item If a local ML model achieve a low accuracy on the reserve dataset, we highlight it as a potential adversary. In the future, we can vary the threshold accuracy to characterize our defense.
\end{enumerate}

\textbf{Quarantine of adversaries}
\begin{enumerate}
    \item Potential adversaries are quarantined, i.e., their ML model parameters are ignored in aggregations. 
\end{enumerate}

\textbf{Aggregation of ML models}
\begin{enumerate}
    \item Aggregate ML models only from those "good" devices. This will readjust the aggregation equation (i.e., the data scaling).
    \item Transmit this completed ML model aggregation to all devices. including adversary devices. 
\end{enumerate}


==> misc.tex <==
Papers to cite:
https://arxiv.org/pdf/2203.04696.pdf - defending against adversaries in FL


==> old_theoretical_results.tex <==
\subsection{Optimality gap of USD-FL} \label{ssec:usd_fl_optimality_gap}
% [motivate theory] 
Because the aggregation rule of USD-FL involves filtering adversarial devices entirely,~\eqref{eq:mod_agg} is effectively training a global model on a sampled subset of training data. %caused by adversarial device filtering
This data sampling effect means that USD-FL will have a performance gap relative to standard FL without any adversaries. 
Since standard FL has been proven theoretically to converge~\cite{wang2019adaptive,dinh2020federated,chen2020convergence} to an optimal set of model parameters $w^{*}$, we can show that, if USD-FL converges to unperturbed standard FL, then USD-FL should by extension also converge to an optimal point. 
% talk about the importance of an optimality gap between USD-FL and theoretical optimal - allude to standard federated learning with no adversaries 

To this end, we first define a common set of assumptions used in literature~\cite{wang2019adaptive,t2020personalized} for general loss functions $\mathcal{L}$: 
\begin{assumption} \label{assumption:lipschitz+strong_convex} We assume that $\mathcal{L}(w)$ is $\rho$-Lipschitz, i.e., $\Vert \mathcal{L}(w) - \mathcal{L}(w') \Vert \leq \rho \Vert w - w' \Vert$ $\forall w, w'$, and $\mu$-strongly convex, i.e., $\mathcal{L}(w') \geq \mathcal{L}(w) + (w'-w)^{T} \nabla \mathcal{L}(w) + \frac{\mu}{2} \Vert w - w' \Vert^2$ $\forall w,w'$. 
\end{assumption}
In Assumption~\ref{assumption:lipschitz+strong_convex}, we use $\mathcal{L}(w)$ to refer to the classification loss of $w$ on the data across all network devices, i.e., $\mathcal{L}(w)= \mathcal{L}(\mathcal{D}_K,w)$ where $\mathcal{D}_K \triangleq \cup_{k \in \mathcal{K}} \mathcal{D}_k$. When we refer to $\mathcal{L}(w)$ on a particular device $k$'s dataset $\mathcal{D}_k$, we will denote it by $\mathcal{L}(\mathcal{D}_k,w)$. In addition, $\mathcal{L}(w)$ retains the properties first described in Sec.~\ref{sec:atk_ovr_method}. 

\begin{lemma} [Gap between USD-FL and standard FL] \label{lemma:std_fl} %trained without any adversarial devices
Given a set of standard FL parameters $\widehat{w}^{t}$, the gap between standard FL and USD-FL is bounded $\forall t$ by: 
\begin{equation} \label{eq:optim_gap_result}
\begin{aligned}
    % &\mathcal{L}(w^{t}) - \mathcal{L}(\widehat{w}^{t}) \leq \left( \frac{\sum_{a \in \mathcal{A}^{t}} w_a D_a} {D_{\mathcal{A}^{t}}}\right)^{T} \nabla \mathcal{L}(w^{t} ) \\
    % &+ \frac{\rho}{2} \left\Vert \frac{\sum_{a \in \mathcal{A}^{t}} w_a D_a} {D_{\mathcal{A}^{t}}} \right\Vert^2,
    % --- expanded form
    % & \mathcal{L}(w^{t}) - \mathcal{L}(\widehat{w}^{t}) \leq \left( \frac{\sum_{k \in \mathcal{K}} \mathds{1}_{\{ \xi^{t}_k < \Xi^{t} \} } w_k D_k} {\sum_{k \in \mathcal{K}} \mathds{1}_{\{ \xi^{t}_k < \Xi^{t} \} } D_k} \right)^{T} \nabla \mathcal{L}(w^{t} ) \\ 
    % & + \frac{\rho}{2} \left\Vert \frac{\sum_{a \in \mathcal{A}^{t}} w_a D_a} {D_{\mathcal{A}^{t}}} \right\Vert^2,
    % --- end expanded form
    % \mathcal{L}(\widehat{w}^{t}) - \mathcal{L}(w^{t}) \leq \zeta(\mathcal{A}^{t})^{T} \nabla \mathcal{L}(w^{t} ) + \frac{\rho}{2} \left\Vert \zeta(\mathcal{A}^{t}) \right\Vert^2, 
    \mathcal{L}(\widehat{w}^{t}) - \mathcal{L}(w^{t}) \leq \zeta(\Xi^{t})^{T} \nabla \mathcal{L}(w^{t} ) + \frac{\rho}{2} \left\Vert \zeta(\Xi^{t}) \right\Vert^2, 
\end{aligned}
\end{equation}
% where $\zeta(\mathcal{A}^{t})\triangleq \sum_{a \in \mathcal{A}^{t}} w_a D_a / {D_{\mathcal{A}^{t}}}$ and $\mathcal{D}_{\mathcal{A}^{t}} \triangleq \cup_{a \in \mathcal{A}^{t}} \mathcal{D}_a$. 
where 
\begin{equation}
\begin{aligned}
    & \zeta(\Xi^{t}) \triangleq \bigg( \sum_{k^{'} \in \mathcal{K}} \mathds{1}_{ \{\xi^{t}_{k^{'}} \geq \Xi^{t} \} } D_{k^{'}} \sum_{k \in \mathcal{K}} w_k D_k \\
    & - \sum_{k \in \mathcal{K}} D_k \sum_{k^{'} \in \mathcal{K}} \mathds{1}_{ \{\xi^{t}_{k^{'}} \geq \Xi^{t} \} } w_{k^{'}} D_{k^{'}} \bigg)  \\
    & \bigg( \sum_{k^{'} \in \mathcal{K}} \mathds{1}_{ \{ \xi^{t}_{k^{'}} < \Xi^{t}\}} D_{k^{'}} \sum_{k \in \mathcal{K}} D_k \bigg)^{-1}.
\end{aligned}
\end{equation}
\end{lemma}
\begin{proof}
Combining the $\rho$-Lipschitz and $\mu$-strongly convex properties of $\mathcal{L}$ and noting that $\widehat{w}^{t} - w^{t}= \zeta(\Xi^{t})$  by definition yields the result. 
\end{proof}

% [give some insight] 
If USD-FL does not set a threshold (i.e., $\Xi^{t} = 0$), then all devices will exhibit $\xi^{t}_k \geq \Xi^{t}$. Correspondingly, $\zeta(\Xi^{t}) \rightarrow 0$ and Lemma~\ref{lemma:std_fl} converges to 0, confirming intuition that USD-FL and standard FL will yield the same result when the set of perceived adversaries is empty (i.e., $\widehat{\mathcal{A}}^{t} = \emptyset$). 
Conversely, if USD-FL sets a galactic threshold (i.e., $\Xi^{t} \rightarrow \infty$), then no device will exhibit $\xi^{t}_k \geq \Xi^{t}$ and the right hand side of~\eqref{eq:optim_gap_result} grows large. 
%In scenarios where USD-FL does not detect any adversaries in the network, the set of adversaries is empty (i.e., $\mathcal{A}^{t} = \emptyset$). Therefore $\zeta({\mathcal{A}^{t}}) \rightarrow 0$ and Lemma~\ref{lemma:std_fl} converges to 0, confirming intuition that USD-FL and standard FL will yield the same result. 

Lemma~\ref{lemma:std_fl} highlights how the gap between USD-FL and standard FL is tightly controlled by $\Xi^{t}$, the adversary detection threshold. USD-FL favors high performing devices with large $\Xi^{t}$, which, on the flip side, can increase the gap to standard FL. We next define a theoretical term in the path to derive the optimality gap of the USD-FL algorithm. %use this gap, alongside an additional theoretical term to derive the optimality of gap of the USD-FL algorithm. 
% Once we define an additional theoretical term, we will use the gap between USD-FL and standard FL in Lemma~\ref{lemma:std_fl} to derive the optimality gap of the USD-FL algorithm.  

\begin{definition} [Gradient loss differential between USD-FL and standard FL] \label{def:grad_diff_usd_fl} 
USD-FL only computes weighted gradients from a subset of the total network datasets. Thus, there is an instantaneous differential between USD-FL and FL gradients, which we define below $\forall t$:  %and gradients computed from all network devices (i.e., FL)
%  We define the instantaneous difference in gradient losses as a result of USD-FL  parameters $w$ and standard FL parameters $\widehat{w}$ as follows:
% \vspace{-2mm}

{\small
\begin{equation} \label{eq:def_grad_error}
\begin{aligned}
    % & e^{t}(w^{t}) = \frac{D_K - D_{\mathcal{Q}^{t}}}{D_K D_{\mathcal{Q}^{t}}} \sum_{q \in \mathcal{Q}^{t}} \nabla \mathcal{L}(\mathcal{D}_q,w^{t}) \\ 
    % & - \frac{1}{D_K} \sum_{a \in \mathcal{A}^{t}} \nabla \mathcal{L}(\mathcal{D}_a,w^{t}), 
    & e^{t}(w^{t}) = \frac{K - \widehat{Q}^{t}}{K \widehat{Q}^{t}} \hspace{-1.5mm} \sum_{q \in \widehat{\mathcal{Q}}^{t}} \hspace{-0.5mm} \nabla \mathcal{L}(\mathcal{D}_q,w^{t}) - \frac{1}{K} \hspace{-1.5mm} \sum_{a \in \widehat{\mathcal{A}}^{t}} \hspace{-0.5mm} \nabla \mathcal{L}(\mathcal{D}_a,w^{t}). \hspace{-1mm}
\end{aligned}
\end{equation}
}
% where $\mathcal{D}_{\widehat{\mathcal{Q}}^{t}} \triangleq \cup_{q \in \widehat{\mathcal{Q}}^{t}} \mathcal{D}_q$ and $\mathcal{D}_{\wide$. % and~\eqref{eq:def_grad_error} is defined $\forall t$. 
\end{definition}

We now have all the tools needed to derive the optimality gap of the USD-FL algorithm. 
\begin{theorem} [Optimality gap of USD-FL] \label{theorem:optim_gap} 
Assuming training step size $\eta \equiv 1/\rho$, the optimality gap of USD-FL is bounded as follows:
% \vspace{-2mm}
{\small
\begin{equation}
\begin{aligned}
    &\mathcal{L}(w^{t+1}) - \mathcal{L}(w^{*}) \leq \mathcal{L}(w^{t}) - \mathcal{L}(w^{*}) \\ 
    & + \frac{\mu}{\rho} \bigg[ \zeta(\Xi^{t})^{T} \nabla \mathcal{L}(w^{t} ) + \frac{\rho}{2} \left\Vert \zeta(\Xi^{t}) \right\Vert^2 \bigg] \\
    & + \frac{\mu}{\rho} \left( 1-\frac{\mu}{\rho} \right) \bigg[  \mathcal{L}(w^{*}) - \mathcal{L}(\widehat{w}^{t-1}) \bigg] + \frac{1}{2\rho} \Vert e^{t}(w^{t})\Vert^2. 
\end{aligned}
\end{equation}
}
\end{theorem}
\begin{proof}
    Since $\mathcal{L}$ is $\mu$-strongly convex, we have:
    \begin{equation} \label{eq:mu_convex}
        \mathcal{L}(w^{t+1}) \geq \mathcal{L}(w^{t}) + (w^{t+1}-w^{t})^{T} \nabla \mathcal{L}(w^{t}) + \frac{\mu}{2} \Vert w^{t+1}-w^{t} \Vert^2. 
    \end{equation}
    Taking the minima of both sides in~\eqref{eq:mu_convex} yields $\mathcal{L}(w^*) \geq \mathcal{L}(w^{t}) - \frac{1}{2\mu} \Vert \nabla \mathcal{L}(w^{t}) \Vert^2$, which after introducing $\mathcal{L}(\widehat{w}^{t})$ to both sides and rearranging yields:
    \begin{equation} \label{eq:lower_grad_bound}
        2\mu \left(\mathcal{L}(w^{t}) - \mathcal{L}(\widehat{w}^{t}) + \mathcal{L}(\widehat{w}^{t}) - \mathcal{L}(w^*) \right) \leq \Vert \nabla \mathcal{L}(w^{t}) \Vert^{2}. 
    \end{equation}
    Since $\eta \equiv 1/\rho$, we can combine the expanded update rule of USD-FL, i.e., $w^{t+1} = w^{t} - \eta (\nabla \mathcal{L}(w^{t}) + e^{t}(w^{t}))$, with Assumption~\ref{assumption:lipschitz+strong_convex} to start bounding $\mathcal{L}(w^{t+1}) - \mathcal{L}({w}^{*})$ as follows:
    % \begin{equation}
    \begin{align}
        & \mathcal{L}({w}^{t+1}) - \mathcal{L}({w}^{*}) \overset{(a)}{\leq} \mathcal{L}({w}^{t}) - \mathcal{L}({w}^{*}) \nonumber \\
        & - \frac{1}{2\rho} \Vert \nabla \mathcal{L}({w}^{t}) \Vert^2 + \frac{1}{2\rho} \Vert e^{t}(w^{t})\Vert^2 \\
        & \overset{(b)}{\leq} \mathcal{L}({w}^{t}) - \mathcal{L}({w}^{*}) \nonumber \\
        & - \frac{\mu}{\rho} \left( \mathcal{L}(w^{t}) - \mathcal{L}(\widehat{w}^{t}) + \mathcal{L}(\widehat{w}^{t}) - \mathcal{L}(w^*) \right) + \frac{1}{2\rho} \Vert e^{t}(w^{t})\Vert^2\\
        & \overset{(c)}{\leq} \mathcal{L}({w}^{t}) - \mathcal{L}({w}^{*}) + \frac{\mu}{\rho} \left( \mathcal{L}(w^*)  - \mathcal{L}(\widehat{w}^{t}) \right) \nonumber \\
        & + \frac{\mu}{\rho} \left( \zeta(\Xi^{t})^{T} \nabla \mathcal{L}(w^{t} ) + \frac{\rho}{2} \left\Vert \zeta(\Xi^{t}) \right\Vert^2 \right) + \frac{1}{2\rho} \Vert e^{t}(w^{t})\Vert^2 \\
        & \overset{(d)}{\leq} \mathcal{L}({w}^{t}) - \mathcal{L}({w}^{*}) + \frac{\mu}{\rho} \left( 1-\frac{\mu}{\rho} \right) \left( \mathcal{L}(w^*)  - \mathcal{L}(\widehat{w}^{t-1}) \right) \nonumber \\
        & + \frac{\mu}{\rho} \left( \zeta(\Xi^{t})^{T} \nabla \mathcal{L}(w^{t} ) + \frac{\rho}{2} \left\Vert \zeta(\Xi^{t}) \right\Vert^2 \right) + \frac{1}{2\rho} \Vert e^{t}(w^{t})\Vert^2, 
    \end{align}
    where $(a)$ is the result of introducing $\mathcal{L}(w^{*})$ to both sides of $\mathcal{L}(w^{t+1}) \leq \mathcal{L}(w^{t}) + (w^{t+1}-w^{t})^{T} \nabla \mathcal{L}(w^{t}) + \frac{\rho}{2} \Vert w^{t+1}- w^{t}\Vert $ (which follows from Assumption~\ref{assumption:lipschitz+strong_convex}) and subsequently combining with the expanded update rule of USD-FL, $(b)$ follows from~\eqref{eq:lower_grad_bound}, $(c)$ uses the result of Lemma~\ref{lemma:std_fl}, and $(d)$ repeats the previous analysis using standard FL parameters $\widehat{w}$ which have a gradient loss differential of $0$ (as standard FL parameters have no differential relative to themselves - see Definition~\ref{def:grad_diff_usd_fl}). 
    %  noting that standard FL uses all of network device datasets and thus incurs no gradient loss difference (i.e., $e^{t}(\widehat{w}^{t}) = 0$). 
    % \end{equation}
\end{proof}


Since $\rho$ is the Lipschitz coefficient, we can always find pairs of $\mu$ and $\rho$ such that $\mu / \rho << 1$. The only remaining step to show that USD-FL converges is to prove that $e^{t}(w^{t})$ is bounded which we demonstrate next. 

\begin{theorem} [Boundedness of $e^{t}(w^{t})$] \label{thm:conv_error} Suppose that device data distributions $\mathcal{D}_k$ have finite second and third moments. Then there exists constants $\gamma_q$ $\forall q \in \widehat{\mathcal{Q}}^{t}$ such that
\begin{equation}
    \Vert e^{t}(w^{t}) \Vert \leq \frac{1}{\widehat{Q}^{t}} \sum_{q \in \widehat{\mathcal{Q}}^{t}} \frac{\gamma_q}{\sqrt{D_q}}.
\end{equation}
\begin{proof}
    Rearranging the definition of $e^{t}(w^{t})$ yields:
    \begin{equation}
        e^{t}(w^{t}) = \frac{1}{\widehat{Q}^{t}} \sum_{q \in \widehat{\mathcal{Q}}^{t}} \nabla \mathcal{L}(\mathcal{D}_q, w^{t}) - \frac{1}{K} \sum_{k \in \mathcal{K}} \nabla \mathcal{L}(\mathcal{D}_k,w^{t}).
    \end{equation}
    Since $\nabla \mathcal{L}(w^{t}) = \frac{1}{K} \sum_{k \in \mathcal{K}} \nabla \mathcal{L}(\mathcal{D}_k,w^{t})$, we can obtain:
    % \begin{equation}
    \begin{align}
        \Vert e^{t}(w^{t}) \Vert & \overset{(a)}{=} \bigg\Vert \frac{1}{\widehat{Q}^{t}} \sum_{q \in \widehat{\mathcal{Q}}^{t}} \nabla \mathcal{L}(\mathcal{D}_q,w^{t})  - \nabla \mathcal{L}(w^{t}) \bigg\Vert \\
        & \overset{(b)}{\leq} \frac{1}{\widehat{Q}^{t}} \sum_{q \in \widehat{\mathcal{Q}}^{t}} \Vert \nabla \mathcal{L}(\mathcal{D}_q,w^{t})  - \nabla \mathcal{L}(w^{t}) \Vert \\
        & \overset{(c)}{\leq} \frac{1}{\widehat{Q}^{t}} \sum_{q \in \widehat{\mathcal{Q}}^{t}} \frac{\gamma_q}{\sqrt{D_q}},
    \end{align}
    % \end{equation}
    where $(a)$ is the definition of $\mathcal{L}(w^{t})$, $(b)$ follows from repeated applications of the triangle inequality, and $(c)$ follows from the central limit theorem by viewing $\nabla \mathcal{L}(\mathcal{D}_q,w^{t}) $ as $D_q$ samples of $\nabla \mathcal{L}(x_d,y_d,w^{t})$ from a distribution with expected value $\nabla \mathcal{L}(w^{t})$. 
\end{proof}
\end{theorem}

As a result of Theorem~\ref{thm:conv_error}, we know that $e^{t}(w^{t})$ is bounded and therefore, via Theorem~\ref{theorem:optim_gap}, USD-FL will converge to an optimal set of parameters with a gap as $t\rightarrow \infty$. As filtering adversaries effectively reduces the data that a global model is trained from, a gap between USD-FL in the presence of adversaries versus unperturbed standard FL is expected. 
We can further verify that there is a gap of USD-FL relative to standard FL when we look at USD-FL convergence in Sec.~\ref{sec:def_eval}. 

% \subsection{Computational Complexity of USD-FL}

% \begin{proposition}[\textbf{Complexity of the Core Defensive Loop in USD-FL}] %Computational Complexity of }]
% \label{prop:complexity}
% Assuming a multi-layer perceptron (MLP) with input dimension $N_I$, a single hidden layer of dimension $N_H$, and output dimension $N_O$, the core defensive loop in USD-FL has complexity: 
% \begin{equation}
%     \mathcal{O}(N_I N_H N_O K C),
% \end{equation}
% where $K$ is the network size, and $C$ is the number of labels. 
% % \mathcal{O}(PKC),
% % where $P = N_iN_hN_O$, $K$ is the network size, and $C$ is the number of labels. 
% \begin{proof}
% The core defensive loop of USD-FL in Algorithm~\ref{alg:usd-fl} relies on the server $S$ to perform an evaluation of local model parameters $w^{t}_k$ for each device $k$.
% This process, outlined in line~\ref{alg_eq:device_acc} of Algorithm~\ref{alg:usd-fl}, involves an indicator over a one-hot matrix of largest dimension $C$, corresponding to the number of unique labels in the dataset, and embeds a set of matrix multiplications between the input dataset and the ML model (assumed to be an MLP for simplicity). 
% The $\argmax$ operation embedded in $\mathds{1}$ will have complexity $\mathcal{O}(C)$, while the MLP model will have $\mathcal{O}(N_I N_H N_O)$ complexity using schoolbook matrix multiplication. Since the defensive loop iterates over the network size $K$, the total complexity is thus $\mathcal{O}(N_I N_H N_O K C)$. 
% % Details about other neural network architectures and their related complexities are in the following Remark. 
% \end{proof}
% \end{proposition}

% \begin{corollary}[\textbf{USD-FL Complexity for Large Models}] \label{coro:complexity}
% Using the same assumptions as Proposition~\ref{prop:complexity}, when we use large ML models (i.e., when $N_I$, $N_H$, and $N_O$ grow large), we can tighten the complexity of USD-FL, obtaining: %we can tighten the complexity of USD-FL for datasets with many unique labels, specifically when $N_I, N_H, N_O$ grow large, and obtain:
% \begin{equation}
%     \mathcal{O}(\max{\{N_I,N_H,N_O\}}^{2.376}KC),
% \end{equation}
% where $K$ is the network size, and $C$ is the number of labels. 
% \begin{proof}
% For datasets with large $N_I$, $N_H$, and $N_O$, padding and subsequent application of galactic algorithms (e.g., Coppersmith-Winograd~\cite{williams2012multiplying}) yields the result. 
% %MLP matrix multiplications can be sped up via padding and subsequent application of galactic algorithms (e.g., Coppersmith-Winograd~\cite{williams2012multiplying}). In the case of Coppersmith-Winograd, this yields the $2.376$ exponential coefficient. 
% \end{proof}
% \end{corollary}

% \begin{remark}[Complexity of USD-FL vs baselines]
% \normalfont
% {\color{blue}something wrong - I need to check this again}
% The computational complexity of baseline defenses for FL is dependent on the ML model architecture, similar to USD-FL. 
% % In particular, coordinate-wise Byzantine defenses (e.g.,~\ref{yin2018byzantine,cao2022mpaf,tao2023byzantine}) 
% In particular, the Median and Trimmed-mean defenses outlined in Fig.~\ref{fig:adv_base_def} rely on a sorting algorithm followed by the application of a coordinate-wise aggregation rule. Assuming the same MLP architecture outlined in Proposition~\ref{prop:complexity} and the use of quicksort~\cite{hoare1962quicksort}, both methods would yield complexity $\mathcal{O}(N_I N_H N_O K\log(K))$. 
% Thus USD-FL is expected to be faster when the network has more devices than unique data labels, i.e., $C < \log(K)$. 
% \end{remark}

% \begin{remark}[ML model architecture and complexity]
% \normalfont
% Complexity of USD-FL and general Byzantine robust FL defenses both depend on the ML model architecture. 
% % For simplicity, 
% We assumed the use of an MLP with a single hidden layer, which only involves linear operators, in Proposition~\ref{prop:complexity} and Corollary~\ref{coro:complexity}, as this captures the essence of the complexity comparison between our methodology and the baseline defenses. 
% For general convolutional neural network (CNN) architectures, one can use the Toeplitz matrix method in~\cite{salehi2022convolution} or the conventional convolutional layer arithmetic in~\cite{dumoulin2016guide}. 
% \end{remark}

